It's About Time: Analog Clock Reading in the Wild

In this paper, we present a framework for reading analog clocks in natural images or videos. Specifically, we make the following contributions: First, we create a scalable pipeline for generating synthetic clocks, significantly reducing the requirements for the labour-intensive annotations; Second, we introduce a clock recognition architecture based on spatial transformer networks (STN), which is trained end-to-end for clock alignment and recognition. We show that the model trained on the proposed synthetic dataset generalises towards real clocks with good accuracy, advocating a Sim2Real training regime; Third, to further reduce the gap between simulation and real data, we leverage the special property of "time", i.e.uniformity, to generate reliable pseudo-labels on real unlabelled clock videos, and show that training on these videos offers further improvements while still requiring zero manual annotations. Lastly, we introduce three benchmark datasets based on COCO, Open Images, and The Clock movie, with full annotations for time, accurate to the minute.

==> latex/06-Applications.tex <==
\section{Applications}

** I don't think we should include this section unless we have demonstrations of any of the examples. Most of it is now mentioned in the intro. If we can read voltmeters, then keep that  **

While being able to tell the time the image is taken is an application in itself, the task of clock reading also has other applications, which are outlined in this section.
\subsection{Time correction in images}
Cameras store the photos’ metadata in the EXIF file, which includes the time the image is taken. However, this is often inaccurate for various reasons, such as when the internal camera’s clock deviates from the real clock by a fixed amount. Moreover, as EXIF does not contain any information on timezones, time differences due to different geographical locations or daylight savings are unable to be corrected.

Given the clock reading, we can verify this time difference that is fixed for each camera, and then re-calibrate them accordingly.

\subsection{Reading instruments}
While the focus on this paper is on analog clocks, it is important to note that clocks are just a (rather difficult) instance of analog scales. Applying this to other type of scales from scientific instruments to industrial gauges is a simple adaptation of our framework.

\begin{comment}
As a simple example, we adapt our framework towards reading voltmeters. To achieve this, we simply adapt our generator to create synthetic voltmeters, and change the 720-way classification (for minute and second) to x-way for voltmeter reading, without changing anything else.

We show in Figure x that our model is easily capable in reading these meters. The same method can be applied to other analog gauges as well, which is a beneficial use case.
\end{comment}

\subsection{Video forensics} 
Being able to tell the time can also provide a cue towards telling whether a video has been edited or not. Video speed manipulation \cite{hosler2020detecting} is sometimes used to change the apparent tone of speakers. 
In fast record attempts such as video game speedrunning, manipulating time by speeding up the video or splicing different segments is prevalent.
In these cases, we know that the rate that time progresses is a constant throughout, and any deviation from that would translate to the video being tampered.
While this ability is currently limited by the presence of clocks, cues from time can be obtained in other ways, such as using optical character recognition models on digital clocks.

\begin{comment}
\section{Digital Clock Reading}
\weidi{Is this section necessary ?}
While this paper focuses on reading analog clocks, we also show that digital clocks can simply be read read using off-the-shelf optical character recognition (OCR) models in Figure \ref{fig:digital}. We utilise the cue that hour and minute are usually separated by a colon (:) in extracting text.

While this method allows clock reading in general, it is not very robust as it relies on the presence of the colon, which does not apply to all clocks. Future work can look into combining this with a detection bounding box and ensuring that the number falls into a certain range.

\begin{figure}[!htb]
\includegraphics[width=\linewidth]{latex/figure/digital.png}
\caption{\textbf{Reading digital clocks.} Digital clocks can be read using off-the-shelf text spotting models. The image shows examples of digital clocks, and the text extracted.}

\centering
\label{fig:digital}
\end{figure}
\end{comment}

==> latex/commented.tex <==

\begin{comment}
\begin{table*}[!htb]
\setlength\tabcolsep{4pt}
\footnotesize
\centering
\begin{tabular}{l|ccccc|ccccc|ccccc}
\toprule
& \multicolumn{5}{c|}{COCO} 
& \multicolumn{5}{c|}{OpenImages} 
& \multicolumn{5}{c}{ClockMovies} \\ \cmidrule{2-16}
Model & TOP1 & TOP1-H  & TOP1-M  & TOP2 & TOP3 & TOP1  & TOP1-H  & TOP1-M  & TOP2 & TOP3 & TOP1 & TOP1-H  & TOP1-M  & TOP2 & TOP3  \\ \midrule
& & & & & & & & & & & & & & \\ \bottomrule  
\end{tabular}
\caption{\textbf{End-to-end recognition results}. 
\weidi{final results, including detection and recognition.}.}
\label{tab:ab1}
\vspace{-5pt}
\end{table*}


\begin{figure}[!htb]
\includegraphics[width=\linewidth]{latex/figure/failure.png}
\caption{\textbf{Failure cases.} We show instances where our model fails. This includes confusion between hands, misleading cues, low resolution, artefacts, generalization gap, and detector failure.}

\centering
\label{fig:failure}
\end{figure}
\end{comment}


\begin{comment}
\subsection{Main results}
\label{sec:main}
%\weidi{fill in this in Table 6, it should be training with different datasets, and benchmark on the datasets that are not trained.}
To our best knowledge, no existing work has been able to achieve success in this setting, so it is challenging to compare to prior work. The results are shown in Table \ref{tab:main_new}. We show that the model is able to achieve success in all these challenging datasets.


\begin{table}[h]
\small
\centering
\begin{tabular}{l|ccccc}
Dataset     & 1 & 1-H & 1-M & 2 & 3 \\ \hline
COCO      & \textbf{66.7} & 74.6 & 73.0 & 69.8 & 74.6  \\
OpenImages      & \textbf{66.7} & 74.6 & 73.0 & 69.8 & 74.6  \\
Clock Movies     & \textbf{54.6} & 57.5 & 63.9 & 62.6 & 67.7\\
\end{tabular}
\caption{\textbf{Main results.} We report the accuracy on the three datasets. 1, 2, 3 represent top 1, 2, and 3 overall accuracies respectively. 1-H and 1-M represent top-1 hour and minute accuracies respectively.}
\label{tab:main_new}
\end{table}

\subsection{Ablation studies}
\label{sec:ablation}
As this is a new task, there are several new components being introduced. We therefore conduct an extensive ablation study to validate the importance of these components.

\begin{table*}[!htb]
\footnotesize
\centering
\begin{tabular}{l|ccccc|ccccc|ccccc}
          & \multicolumn{5}{c|}{COCO} & \multicolumn{5}{c|}{OpenImages} & \multicolumn{5}{c}{Clock Movies}  \\ \hline
Training&  1  & 1-H  & 1-M  & 2 & 3 & 1  & 1-H  & 1-M  & 2 & 3 & 1  & 1-H  & 1-M  & 2 & 3  \\ \hline
SynClock  & -      &   &   &  &  &   &   &   &  &  &   &   &  &  & \\ 
+ Augmentation  & -     &   &   &  &  &   &   &   &  &  &   &   &  &  & \\ 
+ Homography  & -     &   &   &  &  &   &   &   &  &  &   &   &  &  & \\ 
+ Artefacts  & -     &   &   &  &  &   &   &   &  &  &   &   &  &  & \\ \hline
+ Spatial Transformer & -      &   &   &  &  &   &   &   &  &  &   &   &  &  & \\ 
+ Pseudo-label real videos & -     &   &   &  &  &   &   &   &  &  &   &   &  &  & \\ \bottomrule
\end{tabular}
\caption{\textbf{Ablation studies}. We show that augmentation, 
including jittering, blurring, rescaling, homography transform, 
and artefacts (shadows and random lines) are all essential components of our model.}
%\weidi{all experiments should use ResNet50, and 20\% contexts.}}
\label{tab:ab1}
\vspace{-5pt}
\end{table*}


\begin{table*}[]
\small
\centering
\begin{tabular}{l|ccc|ccccc|ccc|ccccc}
            & \multicolumn{8}{c|}{COCO (val)} &  \multicolumn{8}{c}{OpenImages}  \\ \hline
 & mAP& AP50& AP75 &   1  & 1-H  & 1-M  & 2 & 3 & mAP& AP50& AP75 & 1  & 1-H  & 1-M  & 2 & 3  \\ \hline
Detector  & 77.0 & 92.1      & 82.5    & &      & &  & &    61.5 & 89.2 & 66.4   &   &   &  &  & \\ 
GT & \checkmark     &     \checkmark&\checkmark   &  &  &   &   &  & \checkmark     &     \checkmark&\checkmark   & &      &   &   & \\ 
\bottomrule
\end{tabular}
\caption{\textbf{Detection ablations.} To be consistent with the object detection literature, we report the average precisions (AP$_{50}$, AP$_{75}$), where the bounding box IoU is over a threshold. We also report the mean average precision (mAP), which is the average of average precisions across the thresholds [50:5:95]. Overall, the detection task is reasonably successful.}
\label{tab:detection}
\end{table*}

\subsubsection{Synthetic dataset generator}
We test ablating several components of the synthetic dataset generator, as shown in Table \ref{tab:ab1}. 
We start with a basic generator, and show that by incrementally adding (i) augmentation (jittering, blurring and rescaling), (ii) affine transformation, and (iii) artefacts (shadow and random lines) all improve the performance.

\subsubsection{Model architecture}

%\noindent \textbf{Network architecture.} We test the difference in several encoders (ResNet-18, 50, and 101), and surprisingly found that deeper neural networks lead to slightly worse results, suggesting that the bottleneck of the model may lie in generalizablity rather than the ability to learn representations.\\[-8pt] 

%\noindent \textbf{Object detector.} We test with several variations of object detectors with different performances (YOLO-S, YOLO-M, YOLO-L, YOLO-XL). We find that a better object detector is helpful towards the task, which is expected.\\[-8pt]

%\noindent \textbf{Cropping.} We give 10\% context when cropping from a detector by default, and we vary this setting to see if there is a difference in results. We find that too little or too much cropping slightly affects the performance. \\[-8pt]

\noindent \textbf{Ground truth vs off-the-shelf detection.}
We validate the claim that there detection is largely solved, and is not the bottleneck in performance in this model. We report the performance of COCO (validation set only) and Open Images using both ground-truth bounding box and the off-the-shelf detector in table \ref{tab:detection}. We show that the difference in results are marginal. Note that the pre-trained detector is trained on COCO dataset, so the train set of COCO is not usable here for fair comparison. \\[-8pt]


\noindent \textbf{Necessity of STN}.
We show in Table \ref{tab:ab1} that the spatial transformer network offers performance boost to our architecture. \\[-8pt]

\noindent \textbf{Necessity of mixing pseudo-labelled real videos}.
We show in Table \ref{tab:ab1} that training with real videos offers a significant performance improvement.  \\[-8pt]

\end{comment}

\begin{comment}
\section{Future Work}
As this is a new task, there is ample room for future work. 

\textbf{One-stage framework}. One possibility is to unify the architecture into a one-stage framework, training recognition and detection end-to-end instead of having a two-stage model.

\textbf{Training data}. There is also room to close the generalization gap by training using both synthetic and real datasets. It is hoped that with the presence of the synthetic dataset the amount of real data required can be significantly reduced. Another direction is to look at the results as the number of training data varies.

\textbf{Architecture}. The network architecture is currently a simple residual network, and can also be improved -- from using attention modules to spatial transformer-type networks. 

\textbf{Temporal aggregation}. When performing test on video sequences, we also have an additional cue of the temporal ordering. That is, knowing the correct time in one frame allows knowledge of the time in all the frames. This allows aggregation to be performed during inference time to improve the accuracy.

\textbf{Natural cues}. There is also an open question whether one can sense the time from other cues such as the lighting and the extent of shadows, instead of solely relying on clocks. It will be interesting to explore the extent of granularity this task is possible to perform.
\end{comment}
